A Note on Modeling Self-Suspending Time as Blocking Time in Real-Time Systems

This report presents a proof to support the correctness of the schedulability test for self-suspending real-time task systems proposed by Jane W. S. Liu in her book titled "Real-Time Systems" (Pages 164-165). The same concept was also implicitly used by Rajkumar, Sha, and Lehoczky in RTSS 1988 (Page 267) for analyzing self-suspending behaviour due to synchronization protocols in multiprocessor systems.

==> authorea_build/authorea_paper.tex <==

\input{../preamble}

\input{../header}
\paperfalse

\usepackage{tikz}
\usetikzlibrary{arrows}
\usepackage{sansmath}
\tikzset{>=latex}
\usepackage{enumerate}


\begin{document}

\title{A Note on Modeling Self-Suspending Time as Blocking Time in Real-Time Systems\thanks{This paper is supported by DFG, as part of the Collaborative Research Center SFB876 (http://sfb876.tu-dortmund.de/).}}

\author{Jian-Jia Chen\inst{1}, Wen-Hung Huang\inst{1}, and Geoffrey Nelissen\inst{2}}
\institute{TU Dortmund University, Germany\\
Email: jian-jia.chen@tu-dortmund.de, wen-hung.huang@tu-dortmund.de
\and
CISTER/INESC-TEC, ISEP, Polytechnic Institute of Porto, Portugal \\
Email: grrpn@isep.ipp.pt
}


\maketitle
\input{../paper}
\input{../proof2}

\begin{figure}[t]
  \centering
  \input{../figures/example/example-body.tex}
\caption{An illustrative example of the proof.}
\label{fig:example}  
\end{figure}

\bibliography{../bibliography/biblio}{}

\end{document}


==> figures/example/caption.tex <==
An illustrative example of the proof.
\label{fig:example}
  

==> figures/example/size.tex <==
width=800
